On Accelerated Methods for Saddle-Point Problems with Composite Structure

We consider strongly-convex-strongly-concave saddle-point problems with general non-bilinear objective and different condition numbers with respect to the primal and the dual variables. First, we consider such problems with smooth composite terms, one of which having finite-sum structure. For this setting we propose a variance reduction algorithm with complexity estimates superior to the existing bounds in the literature. Second, we consider finite-sum saddle-point problems with composite terms and propose several algorithms depending on the properties of the composite terms. When the composite terms are smooth we obtain better complexity bounds than the ones in the literature, including the bounds of a recently proposed nearly-optimal algorithms which do not consider the composite structure of the problem. If the composite terms are prox-friendly, we propose a variance reduction algorithm that, on the one hand, is accelerated compared to existing variance reduction algorithms and, on the other hand, provides in the composite setting similar complexity bounds to the nearly-optimal algorithm which is designed for non-composite setting. Besides that, our algorithms allow to separate the complexity bounds, i.e. estimate, for each part of the objective separately, the number of oracle calls that is sufficient to achieve a given accuracy. This is important since different parts can have different arithmetic complexity of the oracle, and it is desired to call expensive oracles less often than cheap oracles. The key thing to all these results is our general framework for saddle-point problems, which may be of independent interest. This framework, in turn is based on our proposed Accelerated Meta-Algorithm for composite optimization with probabilistic inexact oracles and probabilistic inexactness in the proximal mapping, which may be of independent interest as well.

==> inexact_oracle/inexact_oracle.tex <==
\section{Accelerated  Meta-algorithm, $(\delta, L)$ - oracles.}
In this section we consider general optimization problem
\begin{equation}
\label{eq:PrStGen}
\min\limits_{x \in \R^d }\{ F\left( x \right):=f\left( x \right)+g\left( x \right)\} .
\end{equation}

Sufficient conditions for convergence Algorithm \ref{alg:highorder_inexact} is presented in Theorem \ref{theoremCATDinexact}.
This proof based on the proof from the article \cite{Bubeck2020} with adding composite part into the proof. Also Theorem \ref{theoremCATDinexact} contains generalization to the case of $ (\delta, L_f) $ - oracle of function $ f (x)$ and $ (\delta, L_g) $ - oracle of function $ g (x)$.

\textbf{Definition} The pair $(f_{\delta, L} (y), \nabla f_{\delta, L} (y))$ is called $(\delta, L)$ - oracle of the function $ f $, if
\begin{equation} \label{def:deltaL}
    0 \leq f(x)-\left(f_{\delta, L}(y)+\left\langle \nabla f_{\delta, L}(y), x-y\right\rangle\right) \leq \frac{L}{2}\|x-y\|^{2}+\delta \text { for all } x \in Q_f
\end{equation}
\textbf{Definition} The pair 
$(f_{\delta, L,\mu} (y), \nabla f_{\delta, L,\mu} (y))$ is called $(\delta, L,\mu)$- oracle of the function $ f $, if
\begin{equation} \label{def:deltaLmu}
     \frac{\mu}{2}\|x-y\|^{2}\leq f(x)-\left(f_{\delta, L,\mu}(y)+\left\langle \nabla f_{\delta, L,\mu}(y), x-y\right\rangle\right) \leq \frac{L}{2}\|x-y\|^{2}+\delta \text { for all } x \in Q_f
\end{equation}
\textbf{Definition} Let $(F_{\delta, L} (x), \nabla F_{\delta, L} (x))$ be a $(\delta, L)$ - oracle of function $F$ at the point $x$, then $\Omega_ {1,\delta, L} \left (F, y, x \right) $ is the following linear function of $y$:
\begin{equation}
    \Omega_{1, \delta, L}\left(F,x, y\right)=F_{\delta, L}(x)+ \langle \nabla F_{\delta, L} (x), y-x\rangle
\end{equation}
%\pd{please unify notation and use $\langle...,...\rangle$ for scalar product everywhere.}

In this part of the article we will assume that $ f (x)$ is equipped with $ (\delta, L_f) $~-oracle and $ g (x)$ has $ (\delta, L_g) $~-oracle. 
%\pd{Do we need this assumption? Is it possible to assume only that there is $ (\delta, L) $ - oracle? Probably for our particular application it is ok to assume both. But for other applications it would be nice to have inexact UM in the full generality.} Let only  $ (\delta, L_f) $ - oracle of function $ f (x)$ and $ (\delta, L_g) $ - oracle of function $ g (x)$ be available to the AM-\ref{alg:highorder_inexact}.
%\pd{I believe it is better to make separate $L$'s for $f$ and for $g$.} Our aim is to prove the convergence of the Algorithm-\ref{alg:highorder_inexact} in this case.


\begin{algorithm} [h!]
\caption{Accelerated Meta-algorithm (AM) p = 1, $(\delta, L)$ - oracles}\label{alg:highorder_inexact}
	\begin{algorithmic}[1]
		\STATE \textbf{Input:} $F = f + g$ --- $\mu_F$-strongly convex,
		
		$H > 0$, $\delta \geq 0,$
		
		$(f_{\delta, L_f}, \nabla f_{\delta, L_f}) : (\R^d \rightarrow \R, \R^d \rightarrow \R^d)$ - $(\delta, L_f)$ --- oracle of $f$, 

		$(g_{\delta, L_g}, \nabla g_{\delta, L_g}) : (\R^d \rightarrow \R, \R^d \rightarrow \R^d)$ - $(\delta, L_g)$ --- oracle of $g$.

		\STATE $A_0 = 0, y_0 = \tilde{x}_0 = x_0$.
		\FOR{ $k = 0$ \TO $k = K- 1$}
		\STATE Choose $y_{k+1}$ from conditions 
% 		\pd{In the first iteration $\tilde{x}_k$ is not defined}
\begin{equation}
\label{prox_step_inexact}
\hspace{-2em} y_{k+1} = \argmin_{y\in \R^d} \left\{
\Omega_{1, \delta, L_f}(f,\tilde{x}_k;y)+g_{\delta, L_g}(y) +\frac{H}{2}\|y-\tilde{x}_k\|^{2} \right\} \,,
\end{equation}
such that %\pd{Shouldn't here be $H$ instead of $L_f$?}
\begin{align}
    \left\|\nabla\left(\Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2\right)+ \nabla g_{\delta,L_g}\left({y}_{k+1}\right)\right\| \leq \nonumber\\
     \frac{H}{4 }\left\|{y}_{k+1}-\tilde{x}_{k}\right\| -2\sqrt{2\delta L_f}\nonumber
\end{align}

		\[
a_{k+1} = \frac{\lambda_{k+1}+\sqrt{\lambda_{k+1}^2+4\lambda_{k+1}A_k}}{2} 
\text{ , } 
A_{k+1} = A_k+a_{k+1}
\text{ , } 
\]
\[
\tilde{x}_k = \frac{A_k}{A_{k + 1}}y_k + \frac{a_{k+1}}{A_{k+1}} x_k. 
		\]
		
\[ 
\lambda_{k+1} = \frac{1}{2H}
\]
		\STATE $x_{k+1} := x_k-a_{k+1} \nabla f_{\delta, L}(y_{k+1}) - a_{k+1}\nabla g_{\delta, L}(y_{k+1})$.
		\ENDFOR
		\RETURN $y_{K}$ 
	\end{algorithmic}	
\end{algorithm}







\begin{theorem} \label{theoremCATDinexact}
Assume that $F(x)$ has $(2\delta,L_f+L_g,\mu)$~-oracle,
$y_k$ --- output of Algorithm~\ref{alg:highorder_inexact} after $k$ iterations for $p = 1$ and $H\ge 2 L_f$. Let the Algorithm~-\ref{alg:highorder_inexact} also use  $ (\delta, L_f) $ - oracle of function $ f (x)$ and $ (\delta, L_g) $ - oracle of function $ g (x)$; and  the auxiliary subproblems \eqref{prox_step_inexact} are solved inaccurately: %\pd{It seems that not everywhere $L$ was changed to $L_f, L_g$. Please check.}
% \vd{Тут нужно  с $L_f$ разобраться, так как в седловых задачах применяется УМ  с $f = 0$, получается нехорошо}
\begin{align} \label{CATD:inexact_criterion}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\leq \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L_f}
\end{align}
    
%\vd{TODO: добавить неточность из леммы 5} 
%\pd1{Здесь не очень понятно, по какой переменной берется градиент в левой части. Кроме того, не очень понятно, что такое $\nabla g_{\delta, L}\left({y}_{k+1}\right)$. Так как это неточная версия функции $g$, то вообще говоря $g_{\delta, L}\left({y}_{k+1}\right)$ может быть не дифференцируемой.}

%\vd{Нужно также потребовать липшицевость градиента функции $g$. Вроде бы только в такой общности нам это в седловых задачах понадобится.}


If $\delta$ is chosen such that 
\begin{equation}\label{CATD:choosedelta}
    \delta \leq  \frac{\varepsilon \mu}{ 32^2 \cdot L_f}
\end{equation}
then
 \begin{equation} \label{speedCATDinexact}
 F(y_k) - F(x_{\ast}) \leq \frac{c_1 H R^2}{k^2} + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k \,,
 \end{equation}
 where  $c_1 = 4$, $R=\|x_0 - x^{\ast}\|$. 

% The auxiliary problems \eqref{prox_step_inexact} 
% %and the minimization problems associated with finding the $ (\delta, L_f) $ - oracle of function $ f (x)$ and $ (\delta, L_g) $ - oracle of function $ g (x)$
% will be solved in
% $$ O(\ln (\varepsilon^{-1})) $$
% to achieve the accuracy $\varepsilon$ in terms of \eqref{speedCATDinexact}. Thus, the final convergence rate of the Algorithm-\ref{alg:highorder_inexact} will be $\sim 1/k^2$.
\end{theorem}



To prove the Theorem \ref{theoremCATDinexact}, we need the following Theorem \ref{thm:MS}, which is based on Theorem 2.1 from \cite{Bubeck2020}.
\begin{theorem} \label{thm:MS}
Let $(y_k)_{k \geq 1}$~--- be a sequence in $\R^d$, and  $(\lambda_k)_{k \geq 1}$~--- a sequence in $\R_+$. Define $(a_k)_{k \geq 1}$ such that $\lambda_k A_k = a_k^2$ and $A_k = \sum_{i=1}^k a_i$. Define also for any $k\geq 0,x_k = x_0 - \sum_{i=1}^k a_i (\nabla f_{\delta, L_{f}}(y_i)+\nabla g_{\delta, L_{g}}(y_i))$ 
%\pd1{Здесь наверное должно быть $\nabla g_{\delta, L}(y_i)$.} \vd{+}
and $\tilde{x}_k := \frac{a_{k+1}}{A_{k+1}} x_{k} + \frac{A_k}{A_{k+1}} y_k$. Finally assume
if for some $\sigma \in [0,1]$ 
\begin{equation} \label{eq:igdrefined}
\|y_{k+1} - (\tilde{x}_k - \lambda_{k+1} (\nabla f_{\delta, L_{f}}(y_{k+1}) + \nabla g_{\delta, L_{g}}(y_{k+1})))\| \leq \sigma \cdot \|y_{k+1} - \tilde{x}_k\| \,,
\end{equation}
then one has for any $x \in \R^d$,
\begin{equation} \label{eq:rate}
F(y_k) - F(x) \leq \frac{ \|x - x_0\|^2}{2 A_k} + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k \,,
\end{equation}
%\yad1{and
%\begin{equation} \label{eq:Alambdatradeoff}
%\sum_{i=1}^k \frac{A_i}{\lambda_i} \|y_i - \tilde{x}_{i-1}\|^2 \leq \frac{\|x^*\|^2}{1-\sigma^2} \,.
%\end{equation}}
%\yad1{Это условие было нужно для поиска $\lambda_k$, в нашем случае $p=1$ они однозначно определены. }
\end{theorem}
To prove this theorem we introduce auxiliaries lemmas based on lemmas 2.2-2.5 and 3.1 from \cite{Bubeck2020}.

Consider a linear combination of gradients:
\[x_k =x_0 - \sum_{i=1}^k a_i (\nabla f_{\delta, L_{f}}(y_i) + \nabla g_{\delta, L_{g}}(y_i))\]
where coefficients $(a_i)_{i\geq1} \geq 0$ and points $(y_i)_{i\geq1}$ is not defined yet. A key observation for such a linear combination of gradients is that it minimizes the approximate lower bound of $F$.

\begin{lemma} \label{lem:basic1}
Let $\psi_0(x) = \frac{1}{2} \|x-x_0\|^2$ and define by induction  $\psi_{k}(x) = \psi_{k-1}(x) + a_{k} \left( \Omega_{1,\delta, L_f}(f, y_{k}, x)+ \Omega_{1,\delta, L_g}(g, y_{k}, x) \right) =\psi_{k-1}(x) + a_{k} \Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)$. Then $x_k =x_0 - \sum_{i=1}^k a_i (\nabla f_{\delta, L_{f}}(y_i) + \nabla g_{\delta, L_{g}}(y_i))$ is the minimizer of $\psi_k$, and 
$\psi_k(x) \leq A_k F(x) + \frac{1}{2} \|x-x_0\|^2$, where $A_k = \sum_{i=1}^k a_i$. 
\end{lemma}
\begin{proof}
Since $\psi_k(x)$ is strongly convex and smooth then expression
\begin{equation}
    \nabla \psi_k (x)=0
\end{equation}
is the criterion of minimum.

The sequence $x_k$ is satisfied
\begin{align}
    \nabla \psi_k (x_k)=\nabla \left(\left[\sum_{i=1}^k a_{i} \Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)\right] + \frac{1}{2} \|x_k-x_0\|^2 \right)=\\
    =\left[\sum_{i=1}^k a_{i} \left( \nabla f_{\delta, L}(y_i) + \nabla g_{\delta, L}(y_i)\right) \right]+x_k-x_0 =0.
\end{align}
Therefore, $x_k$ is a minimizer of the function $\psi_k$

Let's prove now that
\begin{equation}
    \Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)\leq F(x).
\end{equation}
From the definition of $\Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)$  obtain
\begin{equation}
    \Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)=F_{2\delta,  L_f+L_g}(y_{i})+ \la \nabla F_{2\delta,  L_f+L_g} (y_i), x-y_i \ra \leq F(x).
\end{equation}
From $\psi_k(x)=\left[\sum_{i=1}^k a_{i} \Omega_{1,2\delta, L_f+L_g}(F, y_{k}, x)\right] + \frac{1}{2} \|x-x_0\|^2$ we obtain the statement of the theorem.
\end{proof}
The next idea is to produce a <<control sequence>> $(z_k)_{k\geq1}$ demonstrating that $\psi_k$ is not too far below $A_k F$. From this we can directly yield a convergence rate for $z_k$.

\begin{lemma} \label{lem:basic2}
Let $(z_k)$ be a sequence such that 
\begin{equation} \label{eq:tosatisfy}
\psi_k(x_k) - A_k F(z_k) \geq - 2\left(\sum_{i = 1}^k A_{i} \right) \delta\,.
\end{equation}
Then one has for any $x$,
\begin{equation} \label{eq:tosatisfy2}
F(z_k) \leq F(x) + \frac{\|x-x_0\|^2}{2 A_k} + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k  \,.
\end{equation}
\end{lemma}

\begin{proof}
Using Lemma \ref{lem:basic1}) we obtain 
\begin{align}
    A_k F(z_k) \leq \psi_k(x_k) + 2\left(\sum_{i = 1}^k A_{i} \right) \delta \leq \psi_k(x) + 2\left(\sum_{i = 1}^k A_{i} \right) \delta \\
    \leq A_k F(x) +\frac{1}{2}\|x-x_0\|^2 + 2\left(\sum_{i = 1}^k A_{i} \right) \delta \,.
\end{align}
\end{proof}
Our aim now to get sequences $(a_k, y_k, z_k)$, satisfying  \eqref{eq:tosatisfy}.

\begin{lemma} \label{lem:basic3}
One has for any $x,z_k \in \mathbb{R}^d$ and $k\in \mathbb{N}$

%\pd{Думаю, тогда лучше здесь сразу подставить $y_k$, а не $z_k$.} \yad1{Спорно, может возникнуть путанница, что $y_k$ из алгоритма, а в лемме это не используется. Но для меня не принципиально, можно и поменять}
%\pd{Поскольку здесь не принципиален номер у этой произвольной переменной, то лучше заменить на $y$, без $k$.}
\begin{align*}
& \psi_{k+1}(x) - A_{k+1} F(y_{k+1}) - (\psi_k(x_k) - A_k F(z_k)) \\
& \geq A_{k+1} \la \nabla f_{\delta, L_f}(y_{k+1}) +\nabla g_{\delta, L_g}(y_{k+1}),\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1}\ra + \frac{1}{2} \|x -x_k\|^2-2A_{k+1} \delta\,.
\end{align*}
\end{lemma}

\begin{proof}
Firstly from $\Hessian \psi_k (x) = I$ using that $x_k$ is a minimizer of $\psi_k(x)$ we get 
\[
\psi_k(x) = \psi_k(x_k) + \frac{1}{2} \|x- x_k\|^2,\] 
and
\[ \psi_{k+1}(x) = \psi_k(x_k) + \frac{1}{2} \|x-x_k\|^2 + a_{k+1} \Omega_{1, 2\delta, L_f+L_g} (F, y_{k+1}, x) \,,
\]
this,
\begin{equation} \label{eq:ind1}
\psi_{k+1}(x) - \psi_k(x_k) = a_{k+1} \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, x) + \frac{1}{2} \|x-x_k\|^2 \,.
\end{equation}
Now using \eqref{def:deltaL}:
\begin{equation} \label{eq:lem3}
    \Omega_{1,2\delta, L_f+L_g}(F, y_{k+1}, z_k)=F_{2\delta, L_f+L_g}(y_{k+1})+ \la \nabla F_{2\delta, L_f+L_g} (y_{k+1}), 
    z_k-y_{k+1}\ra \leq F(z_k)
\end{equation}
% В полседнем неравенстве пользуемся определением $(\delta,L)$~--- градиента \pd1{Стоит ссылаться на ф-лы, которые используются в выкладках. И лучше расписывать подробнее выкладки, чтобы можно было быстрее проверять, что происходит.}\\
 we obtain:

\begin{eqnarray*}
&&a_{k+1}\Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, x)  =  A_{k+1} \Omega_{1,2\delta, L_f+L_g}(F, y_{k+1}, x)  \\
&-& A_k \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, x) =  A_{k+1} \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, x)   \\
 &-& A_k \la \nabla F_{2\delta, L_f+L_g}(y_{k+1}), x - z_k \ra - A_k \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, z_k)  \\
 & = & A_{k+1} \Omega_{1, 2\delta, L_f+L_g}\left(F, y_{k+1}, x - \frac{A_k}{A_{k+1}} (x - z_k) \right )-  A_k \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, z_k)  \\
 &=& A_{k+1} F_{2\delta, L_f+L_g}(y_{k+1})+  A_{k+1} \la \nabla F_{2\delta, L_f+L_g}(y_{k+1}),\left( x - \frac{A_k}{A_{k+1}} (x - z_k)\right) - y_{k+1}  \ra  \\
 &-& A_k \Omega_{1, 2\delta, L_f+L_g}(F, y_{k+1}, z_k) \stackrel{\eqref{eq:lem3}}{\geq}  A_{k+1} F_{2\delta, L_f+L_g}(y_{k+1}) - A_k F(z_k)\\
 &+ &A_{k+1} \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}),\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1} \ra\\
  &  \stackrel{\eqref{def:deltaL}}{\geq}   & A_{k+1} F(y_{k+1})-2{A_{k+1} \delta} - A_k F(z_k)\\
 &+ &A_{k+1}  \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}),\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1} \ra
 \,,
\end{eqnarray*}
%\vd{Павел, вами было поменяно обозначение скалярного произведения. Это по ошибке или есть причины его поменять во всех местах?}
%\pd{Это специально. Было вразнобой: где-то точка, где-то уголки (в определении неточного оракула например). Поскольку в других частях статьи тоже уголки, то нужно везде поменять на уголки.}
which concludes the proof.

% \begin{eqnarray*}
% & &a_{k+1}\Omega_{1, \delta, L}(F, y_{k+1}, x)  =  A_{k+1} \Omega_{1,\delta, L}(F, y_{k+1}, x) - A_k \Omega_{1, \delta, L}(F, y_{k+1}, x) \\
% & = & A_{k+1} \Omega_{1, \delta, L}(F, y_{k+1}, x) - A_k  F_{\delta, L}(y_{k+1}) \cdot (x - z_k) - A_k \Omega_{1, \delta, L}(F, y_{k+1}, z_k) \\
%  & = & \left( A_{k+1} \Omega_{1, \delta, L}\left(F, y_{k+1}, x - \frac{A_k}{A_{k+1}} (x - z_k) \right ) \right) - \left\{ A_k \Omega_{1, \delta, L}(F, y_{k+1}, z_k)\right\} \\
%  & \geq &  (A_{k+1} (\nabla f_{\delta, L}(y_{k+1})+\nabla g_{\delta, L}(y_{k+1})) \cdot \left(\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1} \right) +\\
%  & + & A_{k+1} F_{\delta,L}(y_{k+1}))  - \left\{ A_k F(z_k) \right\} \\
%  \end{eqnarray*}
%  В последнем неравенстве воспользовались оценкой \eqref{eq:lem3}.
 
%  Используя то, что $F(x) \leq F_{\delta, L}(x) + \delta$ из \eqref{def:deltaL}, получим:
%  \begin{eqnarray*}
% &  & (A_{k+1} (\nabla f_{\delta, L}(y_{k+1})+\nabla_{\delta, L} g(y_{k+1})) \cdot \left(\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1} \right) +\\
%  & + & A_{k+1} F_{\delta,L}(y_{k+1}))  - \left\{ A_k F(z_k) \right\} \geq\\
%   & \geq  & A_{k+1} F(y_{k+1})-\vd{A_{k+1} \delta} - A_k F(z_k)\\
%  &+ &A_{k+1} (\nabla f_{\delta, L}(y_{k+1})+\nabla g_{\delta, L}(y_{k+1})) \cdot \left(\frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} z_k - y_{k+1} \right )
%  \,,
% \end{eqnarray*}
% % \pd1{В разных местах скалярное произведение записано по-разному. Это очень запутывает.}
% % \vd{Поправили}
% что завершает доказательство.

\end{proof}

\begin{lemma} \label{lem:basic4}
Denoting  
\begin{equation}\label{eq:lambda}
    \lambda_{k+1} := \frac{a_{k+1}^2}{A_{k+1}}
\end{equation}
 and $\tilde{x}_k := \frac{a_{k+1}}{A_{k+1}} x_{k} + \frac{A_k}{A_{k+1}} y_k$, one has:
\begin{align*}
& \psi_{k+1}(x_{k+1}) - A_{k+1} F(y_{k+1}) - (\psi_k(x_k) - A_k F(y_k)) \geq \\
& \frac{A_{k+1}}{2 \lambda_{k+1}} \bigg( \|y_{k+1} - \tilde{x}_k\|^2 - \|y_{k+1} - (\tilde{x}_k - \lambda_{k+1} (\nabla f_{\delta, L_f}(y_{k+1}))+\nabla g_{\delta, L_g}(y_{k+1})) \|^2 \bigg) - 2A_{k+1} \delta \,.
\end{align*}
In particular, we have in light of \eqref{eq:igdrefined}
$$\psi_{k}(x_{k})-A_{k}F(y_{k})\geq\frac{1-\sigma^{2}}{2}\sum_{i=1}^{k}\frac{A_{i}}{\lambda_{i}}\|y_{i}-\tilde{x}_{i-1}\|^{2} - 2\left(\sum_{i = 1}^k A_{i} \right) \delta.$$
\end{lemma}

\begin{proof}
We apply Lemma \ref{lem:basic3} with $z_k = y_k$ and $x=x_{k+1}$ 
%\pd{я так понял, это не используется} \yad1{Вроде все ок}
, and 
note that (with $\tilde{\xi} := \frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} y_k$): 
% \pd{Тут какая-то путаница. В алгоритме 1 и условии теоремы $\tilde{x}$ определяется через $x_k$. То есть нужно брать в качестве $x$ $x_k$. Но далее  в качестве $x$ берется $x_{k+1}$. То есть кажется, что в одном месте в качестве $x$ берется $x_{k}$, а в другом в качестве $x$ берется $x_{k+1}$ }
% \yad1{Вроде в этом месте нет ошибок: думаю, что вы ошибочно предполагаете, что $\tilde{x}=\tilde{x}_k$, но это разные вещи ($\tilde{x}$ действительно определяется через $x_{k+1}$, а $\tilde{x}_k$ определяется через $x_{k}$) }
% \pd{Тогда лучше какой-то другой буквой обозначать $\tilde{x}$.}
% \yad1{Исправил на $\tilde{\xi}$}
\begin{align*}
& \la \nabla_{\delta, L_f} f(y_{k+1})+ \nabla g_{\delta, L_g}(y_{k+1}), \frac{a_{k+1}}{A_{k+1}} x + \frac{A_k}{A_{k+1}} y_k - y_{k+1} \ra  + \frac{1}{2 A_{k+1}} \|x - x_k\|^2 \\
& = \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}), \tilde{\xi} - y_{k+1}\ra  + \frac{1}{2 A_{k+1}} \left\|\frac{A_{k+1}}{a_{k+1}} \left(\tilde{\xi} - \frac{A_k}{A_{k+1}} y_k \right) - x_k \right\|^2 \\
& = \la \nabla_{\delta, L_f} f(y_{k+1})+\nabla g_{\delta, L_g} (y_{k+1}), \tilde{\xi} - y_{k+1} \ra + \frac{A_{k+1}}{2 a_{k+1}^2} \left\|\tilde{\xi} - \left(\frac{a_{k+1}}{A_{k+1}} x_k + \frac{A_k}{A_{k+1}} y_k \right) \right\|^2 \,.
\end{align*}

This yields, using \eqref{eq:lambda}:
\begin{align*}
& \psi_{k+1}(x_{k+1}) - A_{k+1} F(y_{k+1}) - (\psi_k(x_k) - A_k F(y_k)) \\
& \geq A_{k+1} \cdot  \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1})), \tilde{\xi} - y_{k+1}) \ra + \frac{A_{k+1}}{2 \lambda_{k+1}} \|\tilde{\xi} - \tilde{x}_k\|^2  -2 A_{k+1} \delta\\
& \geq A_{k+1} \cdot \min_{x \in \R^d} \left\{ \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}), x - y_{k+1}\ra  + \frac{1}{2 \lambda_{k+1}} \|x - \tilde{x}_k\|^2 \right\} -2 A_{k+1} \delta\,.
\end{align*}
The value of the minimum is easy to compute. Due to the strong convexity of the minimized function and its continuous differentiability, achieving a minimum is equivalent to the condition
\begin{align*}
    & 0=\nabla \left[ \la \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta,L_g}(y_{k+1}), x - y_{k+1} \ra + \frac{1}{2 \lambda_{k+1}} \|x - \tilde{x}_k\|^2\right]=\\
    & =(\nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1})) + \frac{1}{ \lambda_{k+1}} \left( x - \tilde{x}_k\right) 
\end{align*}
Then
\begin{align*}
    x_{*}= \tilde{x}_k-\lambda_{k+1}(\nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1})) 
\end{align*}
Substituting into the last inequality we obtain the statement of the theorem.

%\pd{Лучше добавить детали.} \yad1{Done}
%\pd{Проведите еще, пожалуйста, выкладку с подстановкой. Я не понимаю, откуда там в квадратичных членах $y_{k+1}$ возникает.}
%\yad1{Done!
%Это легче сделать, если начать расписывать то, что нужно доказать:
%\begin{align*}
%&\frac{A_{k+1}}{2 \lambda_{k+1}} \bigg( \|y_{k+1} - \tilde{x}_k\|^2 - \|y_{k+1} - (\tilde{x}_k - \lambda_{k+1} (\nabla f_{\delta, L_f}(y_{k+1}))+\nabla g_{\delta, L_g}(y_{k+1})) \|^2 \bigg) - \vd{2A_{k+1} \delta} \\
%&=\frac{A_{k+1}}{2 \lambda_{k+1}} \bigg(2 \lambda_{k+1} \la  \nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}), y_{k+1} - \tilde{x}_k \ra -\\ &- \|\lambda_{k+1} (\nabla f_{\delta, L_f}(y_{k+1})+\nabla g_{\delta, L_g}(y_{k+1}))\|^2 \bigg) - \vd{2A_{k+1} \delta}
%\end{align*}
%Тут уже нет квадратичных членов, в точности это и получится, если подстановку сделать.
%}

\end{proof}
\begin{proof} \textbf{of the Theorem \ref{thm:MS}}

Using Lemma \ref{lem:basic4} we get
$$\psi_{k}(x_{k})-A_{k}F(y_{k})\geq\frac{1-\sigma^{2}}{2}\sum_{i=1}^{k}\frac{A_{i}}{\lambda_{i}}\|y_{i}-\tilde{x}_{i-1}\|^{2} - 2\left(\sum_{i = 1}^k A_{i} \right) \delta \geq - 2\left(\sum_{i = 1}^k A_{i} \right) \delta.$$
Applying Lemma \ref{lem:basic2} for $z_k=y_k$ one has for any $ x \in \mathbb{R}^d$:
\begin{equation} 
F(y_k) - F(x) \leq \frac{ \|x-x_0\|^2}{2 A_k} + 2\left(\sum_{i = 1}^k A_{i} \right) \delta /A_k \,,
\end{equation}
\end{proof}
For the first conclusion in Theorem \ref{thm:MS} it suffices to combine Lemma \ref{lem:basic4} with Lemma \ref{lem:basic2} and Lemma 2.5 from \cite{Bubeck2020}.
The second conclusion in Theorem \ref{thm:MS} follows from \ref{lem:basic4} and Lemma \ref{lem:basic1}.






% \pd{Алгоритм 1 надо бы привести к тому виду, который анализируется. Во-первых все-таки его нужно расписать в конкретнос случае $p=1$ (см. \url{https://www.overleaf.com/6774351872zbsbqgttvyxj}. Во-вторых, в (6) используются теперь неточные градиенты. И аналогично на шаге 5.}
% \pd{У нас теперь две неточности. 1я связана с тем, что нам не доступны точные градиенты и сама модель в (6) неточная. 2я связана с тем, что эту неточную модель мы минимизируем неточно. Нужно показать две вещи: что нам действительно доступен $\delta,L$-оракул и что неточную модель мы можем отминимизировать так, чтобы получить (12). Точнее, думаю, лучше на (18) ориентироваться.}
% \yad1{(18) используется как раз для того, чтобы получить (12), поэтому скорее стоит все-таки ориентироваться на (12), мб я что-то не так понял}

Now one will formulate the sufficient condition \eqref{eq:New_inexact} for the accuracy of solving auxiliary problems \eqref{prox_step_inexact}.
%, but to check this condition, exact values of functions $f,g$ are required. Consequently, the validity of this condition cannot be verified by the algorithm directly, since it knows only $f_{\delta,L},\nabla f_{\delta,L},g_{\delta,L},\nabla g_{\delta,L}$. Later one will formulate the new sufficient condition based on \eqref{eq:inexact}, that can already be checked by the algorithm.
Let's assume, that auxiliary problems \eqref{prox_step_inexact} can not be solved exactly. Let the algorithm only have an inaccurate solution ${y}_{k+1}$ satisfying %\pd{Can we take $H$ here instead of $L_f$?}
%\begin{align}\label{eq:New_inexact}
%        &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+L_f\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
%    &\leq \min \lbrace \frac{1}{2}, \frac{L_f}{4\left[ L_f +2L_f \right]} \rbrace \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)-\left(2+\frac{L_f}{\left[ L_f+2L_f \right]}\right)\sqrt{2\delta L}
%\end{align}
\begin{align}\label{eq:New_inexact}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\leq \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L_f}
\end{align}
% \pd{Мы ведь теперь в (6) минимизируем неточную модель, так как точная нам недоступна. Получается некоторая путаница, так как в алгоритме $y_{k+1}$ определяется как неточный минимум неточной модели, а здесь $y_{k+1}$ неточный минимум точной модели. А обозначение одинаковое.}
% \yad1{Тут не должно быть никакой путанницы, все последовательности определяются при работе УМ с неточными моделями и неточным решением вспомогательной задачи. То есть $y_{k+1}$ определяется как неточный минимум неточной модели. В этом вы правы. А дальше идет уже не правда: в последнем неравенстве $y_{k+1}$ тоже является неточным минимумом неточной модели, думаю вас спутало, что условие на точность решения ЗАДАЧИ С НЕТОЧНЫМИ МОДЕЛЯМИ содержит ТОЧНЫЕ значения функций и их градиенты, да, это действительно будет условием остановки при решении ЗАДАЧИ С НЕТОЧНЫМИ МОДЕЛЯМИ. Единственная проблема, что его нельзя проверить при работе УМ с неточными моделями и неточным решением, но она была учтена за счет (18)}
% \pd{Да, меня именно это запутало. Я думаю, что лучше условие для неточного решения задачи с неточной моделью записывать через неточные градиенты. То есть в алгоритме сразу прописывать условие на неточность, которое можно проверить. Это вроде как \eqref{eq:New_inexact}.}
in this case:











\begin{lemma} \label{lem:controlstepsize}
Assume that $f(x)$ has $(\delta,L_f)$~-oracle, $g(x)$ has $(\delta,L_g)$~-oracle and one has the solution of the auxiliary problem \eqref{prox_step_inexact} with the accuracy \eqref{eq:New_inexact}.If 
$$H\geq 2L_f$$ then equation \eqref{eq:igdrefined} holds true with $\sigma = 7/8$ for \eqref{prox_step_inexact}. In the case $p = 1$ one can consider $\lambda_{k+1} = \lambda =  \frac{1}{2H}$.
\end{lemma}
\begin{proof}
%Let's define the sequence:
%\begin{equation}
%\Xi_{k+1}=\nabla\left(\Omega_{1}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+L_{f}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2+g\left({y}_{k+1}\right)\right)
%\end{equation}


Using that $f$ is equipped with a $(\delta, L_f)$~-oracle and Corollary 4.2. from \cite{OlivierDevolder} one obtains:% \pd{It seems that the l.h.s. is 0.}
\begin{equation}\label{eq:speedstrongconvex}
\|\nabla f_{\delta, L_f}(y) - \nabla_y \Omega_{1, \delta, L_f}(f,x, y)\| \leq L_f \|y - x\| + 2\sqrt{2 L_f\delta} \,.
\end{equation}
By \eqref{eq:New_inexact} and \eqref{eq:speedstrongconvex} we can get next inequalities:
\begin{align*}
& \|y_{k+1} - (\tilde{x}_k - \lambda_{k+1} (\nabla_{\delta, L_f} f(y_{k+1})+ \nabla g_{\delta, L_g}(y_{k+1}))) \| \\
&= \|y_{k+1} \pm\lambda_{k+1} \nabla_y \Omega_{1,\delta ,L_f}(f, \tilde{x}_k, y_{k+1})\pm H \lambda_{k+1} (y_{k+1}-\tilde{x}_k) \\
&- (\tilde{x}_k - \lambda_{k+1} (\nabla_{\delta, L_f} f(y_{k+1})+ \nabla g_{\delta, L_g}(y_{k+1}))) \| \leq (1-H \lambda_{k+1})\|(y_{k+1}-\tilde{x}_k)  \|\\
&+ \lambda_{k+1}\| \nabla_y \Omega_{1,\delta ,L_f}(f, \tilde{x}_k, y_{k+1}) + H (y_{k+1} - \tilde{x}_k) + \nabla g_{\delta, L_g}(y_{k+1})\| \\
&+ \lambda_{k+1} \|\nabla_{\delta, L_f} f(y_{k+1})- \nabla_y \Omega_{1,\delta, L_f}(f, \tilde{x}_k, y_{k+1}) \| \stackrel{\eqref{eq:New_inexact},\eqref{eq:speedstrongconvex}}{\leq}  (1-H \lambda_{k+1})\|y_{k+1}-\tilde{x}_k \| \\
& +\lambda_{k+1}\frac{H}{4 }\left\|{y}_{k+1}-\tilde{x}_{k}\right\| -2 \lambda_{k+1} \sqrt{2L_f\delta}+  \lambda_{k+1} \left(L_f \|{y}_{k+1}-\tilde{x}_{k}\| + 2 \sqrt{2 L_f\delta} \right)  \\
&\leq  \left(\frac{5}{8}+\frac{L_f}{2H}\right)\|y_{k+1}-\tilde{x}_k  \|
 \leq \frac{7}{8}\|y_{k+1}-\tilde{x}_k  \|
\end{align*}
that ends the proof.
\end{proof}

To prove Theorem \ref{theoremCATDinexact}, it remains to show that the fulfillment of condition \eqref{eq:New_inexact} keep the linear rate of convergence when solving the auxiliary problems \eqref{prox_step_inexact}.\\
Based on \eqref{eq:New_inexact} we try to relate the accuracy $\tilde{\varepsilon}$ we need to solve \eqref{eq:problem}. For this we prove the auxiliary lemma for $(\delta,L_f)$~-oracle of $f$ and $(\delta,L_g)$~-oracle of $g$, that is based on the Lemma 2.1 from \cite{Grapiglia2019} . 
%\pd{Why this Lemma implies that \eqref{eq:inexact} follows from \eqref{eq:New_inexact}? Or do we now use %\eqref{eq:lemSufficCondit1} as a stopping criterion of the inner algorithm?} 
%\yad1{Тут вы торопитесь, напрямую эта лемма ничего не дает, она будет применяться в следющей лемме чуть в другом виде}
\begin{lemma}\label{lem:SufficConditForStop}
Let $\tilde{x}_k \in \mathbb{R}^d, H,\Theta >0$.\\
Assume that $f(x)$ has $(\delta,L_f)$~-oracle, $g(x)$ has $(\delta,L_g)$~-oracle. If
\begin{align}\label{eq:lemSufficCondit1}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\leq \min \lbrace \frac{1}{2}, \frac{\Theta}{2\left[ L_f +H \right]} \rbrace \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)
\end{align}
then $y_{k+1}$ satisfies 
\begin{align}\label{eq:lemSufficConditRes}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\leq \Theta \|y_{k+1} - \tilde{x}_k\|+\frac{2 \Theta}{\left[ L_f+H\right]}\sqrt{2 L_f\delta}
\end{align}
\end{lemma}
\begin{proof}
Using that $f$ is equipped with a $(\delta, L_f)$~-oracle and Corollary 4.2. from \cite{OlivierDevolder} one obtains:
\begin{equation}\label{eq:lemSufficCondit2}
\|\nabla f_{\delta, L_f}(y) - \nabla_y \Omega_{1, \delta, L_f}(f,x, y)\| \leq L_f \|y - x\| + 2\sqrt{2 L_f\delta} \,.
\end{equation}
Combining \eqref{eq:lemSufficCondit1} and \eqref{eq:lemSufficCondit2} we obtain
\begin{align*}
    &\|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\| \\
    &\leq\|\nabla f_{\delta,L_f} (y_{k+1})+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)-\nabla g_{\delta,L_g}\left({y}_{k+1}\right)-\nabla \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)\| \\
    &+\|\nabla \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)\pm \nabla g_{\delta,L_g}\left({y}_{k+1}\right)-\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)\|\\
    &+\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\stackrel{\eqref{eq:lemSufficCondit2},\eqref{eq:lemSufficCondit1}}{\leq} \left( L_f \|y_{k+1} - \tilde{x}_k\| + 2\sqrt{2 L_f\delta} \right) + H\|y_{k+1} - \tilde{x}_k\| +\\
    &\frac{1}{2}\|\nabla f_{\delta,L_f} (y_{k+1})+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|
\end{align*}
Thus,
\begin{equation}
    \frac{\|\nabla f_{\delta,L_f} (y_{k+1})+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|}{2}\leq \left[ L_f+H\right]\|y_{k+1} - \tilde{x}_k\|+2\sqrt{2 L_f\delta}
\end{equation}
which gives
\begin{equation}\label{eq:lemSufficCondit3}
    \frac{\Theta }{2\left[ L_f+H\right]}\|\nabla f_{\delta,L_f} (y_{k+1})+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\leq \Theta \|y_{k+1} - \tilde{x}_k\|+\frac{2 \Theta}{\left[ L_f+H\right]}\sqrt{2 L_f\delta}
\end{equation}
Finally, \eqref{eq:lemSufficConditRes} follows directly from the \eqref{eq:lemSufficCondit1} and \eqref{eq:lemSufficCondit3}
\end{proof}


















Assume that $f(x)$ has $(\delta,L_f)$~-oracle, $g(x)$ has $(\delta,L_g)$~-oracle.

\begin{lemma} \label{lem:ff}
Assume that $H\geq 2 L_f$, $f(x)$ has $(\delta,L_f)$~-oracle, $g(x)$ has $(\delta,L_g)$~-oracle, $F(x)$ has $(2\delta,L_f+L_g,\mu)$~-oracle; ${y}_{k+1},\tilde{x}_k \in \mathbb{R}^d$ and $\varepsilon \in (0,1)$. If inequalities 
%\pd{If we have an opposite inequality, does it mean that we have an $\varepsilon$-optimal solution?}
%\yad1{It depend on how we will choose the delta, for small enough once the preceding statement is true.}
%\pd{Получается, нужно как-то по ходу итераций это неравенство гарантировать. Если бы все было точно, то это легко: если это неравенство не выполняется, то значит мы нашли решение. А вот в случае неточности, вопрос, как по ходу итераций это неравенство гарантировать. И что такое $Q_f$?}
%\yad1{Тут мы же сами выбираем дельта(это даже сделано в этой теореме) и мы его берем достаточно маленьким (меньше, чем $\frac{\varepsilon}{2}$), поэтому тут нет никаких сложностей, если это условие не выполняется, то значит у нас есть решение с точностью $\varepsilon+\delta$ и можно завершать алгоритм}
\begin{equation}\label{eq:lemmffF}
    \varepsilon\leq F_{2\delta, L_f+L_g,\mu}(y)-\min_{x \in Q_f} F(x)
\end{equation}
\begin{equation}\label{eq:lemmffDelta}
    \delta\leq \frac{\varepsilon \mu}{ 32^2 \cdot L_f},
\end{equation}
is satisfied then inequality \eqref{eq:New_inexact} would hold true if one solve the auxiliary problem  \eqref{prox_step_inexact} with the accuracy 
\begin{equation}\label{eq:lemmffEpsil}
    \tilde{\varepsilon}=O\left( \varepsilon^{\frac{1}{2}} \mu_F^{\frac{1}{2}}\right)
\end{equation}
in terms of criteria \eqref{eq:New_inexact}.
\end{lemma}
\begin{proof}
According to the conditions of the lemma, the problem \eqref{prox_step_inexact} is solved with the accuracy
\begin{equation}
    \|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\leq \tilde{\varepsilon}
\end{equation}
To prove the lemma, it suffices to show the following chain of inequalities
\begin{align}\label{eq:lemff1}
    & \tilde{\varepsilon} \leq \min \lbrace \frac{1}{2}, \frac{H}{8\left[ L_f +H \right]} \rbrace \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)-\left(2+\frac{H}{2\left[ L_f+H \right]}\right)\sqrt{2\delta L_f} \\
    &\leq \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L_f}
\end{align}
Lemma \ref{lem:SufficConditForStop} for $\Theta=\frac{L_f}{2}$ guarantee that if the next inequality holds true
\begin{align}\label{eq:lemff2}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\| \\
    &\leq \min \lbrace \frac{1}{2}, \frac{H}{8\left[ L_f +H \right]} \rbrace \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)-\left(2+\frac{H}{2\left[ L_f+H \right]}\right)\sqrt{2\delta L_f} 
\end{align}
then the equation \eqref{eq:New_inexact} is satisfied.\\
If \eqref{eq:lemff2} is sufficient condition for \eqref{eq:New_inexact}, it means that right-hand sides of \eqref{eq:lemff2} less the right-hand sides of \eqref{eq:New_inexact}. From this consequence the next inequality\\
%\yad1{If \eqref{eq:lemff2} is sufficient condition for \eqref{eq:lemff1},it mean that right-hand sides of \eqref{eq:lemff2} less the right-hand sides of \eqref{eq:lemff1}. From this consequence the next inequality}
%\pd{How \eqref{eq:lemff2} can be sufficient condition for \eqref{eq:lemff1} if \eqref{eq:lemff2} is obtained from \eqref{eq:lemff1}? This transition is still not clear.}
%\yad1{Я когда отвечал случайно перепутал уравнения местами, в доказательство вроде нет ошибки: из выполнения \eqref{eq:lemff2} следует \eqref{eq:New_inexact}, поэтому правая часть \eqref{eq:lemff2} меньше правой части \eqref{eq:New_inexact}}
\begin{align}
    &\frac{1}{12} \left( \|\nabla F_{2\delta,L_f+L_g} (y_{k+1}) \|\right)-\frac{5}{2}\sqrt{2\delta L_f} = \frac{1}{12} \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)-\frac{5}{2}\sqrt{2\delta L_f} \\
    &\leq \min \lbrace \frac{1}{2}, \frac{H}{8\left[ L_f +H \right]} \rbrace \left( \|\nabla f_{\delta,L_f} (y_{k+1}) +\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\right)-\left(2+\frac{H}{2\left[ L_f+H \right]}\right)\sqrt{2\delta L_f}  \\
    &\leq  \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L_f} \label{eq:lemff5}
\end{align}
The second inequality of the equation \eqref{eq:lemff1} is satisfied, let's prove the first one.\\
The fact that F has $(2\delta,L_f+L_g,\mu)$~-oracle guarantee
\begin{equation}\label{eq:lemmff3}
     \frac{\mu}{2}\|x-y\|^{2}+\left(F_{2\delta, L_f+L_g,\mu}(y)+\left\langle \nabla F_{2\delta, L_f+L_g,\mu}(y), x-y\right\rangle\right)\leq F(x) \text { for all } x \in Q_f
\end{equation}
Let us minimize the right- and left-hand sides of \eqref{eq:lemmff3} with respect to x independently
\begin{align}
    &F^*=\min_{x \in Q_f} F(x) \stackrel{\eqref{eq:lemmff3}}{\geq} F_{2\delta, L_f+L_g,\mu}(y)+
    \min_{x \in Q_f}\left\{ \frac{\mu}{2}\|x-y\|^{2}+\left\langle \nabla F_{2\delta, L_f+L_g,\mu}(y), x-y\right\rangle\right\}\\
    &=F_{2\delta, L_f+L_g,\mu}(y)-\frac{1}{2\mu} \|\nabla F_{2\delta, L_f+L_g,\mu}(y)\|^2
\end{align}
Then obtain
\begin{equation}\label{eq:lemmff4}
    \varepsilon\stackrel{\eqref{eq:lemmffF}}{\leq} F_{2\delta, L_f+L_g,\mu}(y)-F^* \leq \frac{1}{2\mu} \|\nabla F_{2\delta, L_f+L_g,\mu}(y)\|^2
\end{equation}
Inequality \eqref{eq:lemmff4} guarantee that 
\begin{equation}\label{eq:lemmff6}
    \frac{1}{2}\sqrt{\frac{\varepsilon \mu}{18}} -\frac{5}{2} \sqrt{2\delta L_f}\leq \frac{1}{12} \|\nabla F_{2\delta, L_f+L_g,\mu}(y)\|-\frac{5}{2} \sqrt{2\delta L_f}
\end{equation}
%\begin{align}\label{eq:lemff7}
%    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+L_f\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
%    &\leq \frac{1}{2}\sqrt{\frac{\varepsilon \mu}{18}} -\frac{7}{3} \sqrt{2\delta L}\leq \frac{1}{12} \|\nabla F_{2\delta, L_f+L_g,\mu}(y)\|-\frac{7}{3} \sqrt{2\delta L}\\
%    &\leq \frac{L_f}{2} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L}
%\end{align}
In case of \eqref{eq:lemmffDelta} inequality \eqref{eq:lemmff6} give us guarantees that the first inequality of the equation \eqref{eq:lemff1} holds true
\begin{equation} \label{inexact_precision}
    \tilde{\varepsilon}=\frac{\sqrt{2\varepsilon \mu}}{64}\stackrel{\eqref{eq:lemmffDelta}}{\leq} \frac{1}{2}\sqrt{\frac{\varepsilon \mu}{18}} -\frac{5}{2} \sqrt{2\delta L_f}  \stackrel{\eqref{eq:lemmff6}}{\leq} \frac{1}{12} \|\nabla F_{2\delta, L_f+L_g,\mu}(y)\|-\frac{5}{2} \sqrt{2\delta L_f}
\end{equation}
Finally, combine the equations \eqref{eq:lemff5} and \eqref{inexact_precision} obtain the required chain of inequalities \eqref{eq:lemff1}.
%\pd{it is not clear, what is meant by "in terms of criteria \eqref{eq:New_inexact}"  since \eqref{eq:New_inexact} does not contain any $\varepsilon$.}\\
%\yad1{Да, согласен, что это может быть не понятно. Тут я вижу одно возможное решение: ввести новое неравенство, где будет $\varepsilon$, но у меня такое ощущение, что это избыточно и читатель может запутаться, а так мы ссылаемся на \eqref{eq:New_inexact}, которое уже использовалось в прошлых леммах и появляется какая-то связка. Я могу не видеть друго, более хорошего решения}
%\pd{Получается в итоге не очень понятно, какое условие проверяется непосредственно в алгоритме. Я понимаю, что сейчас логика построена так, что мы знаем, что нам нужно и пытаемся получить условие, которое можно проверить и которое даст нам то, что нужно. Поскольку теперь мы поняли, что это за условие, то можно логику изложения перевернуть. Вот такое условие мы проверяем в алгоритме, вот такое требование у нас на $\delta$, вот такие мы из них получаем следствия и в конце получаем \eqref{eq:igdrefined}, которое нам нужно для сходимости метода.}












\end{proof}
















% Заметим, что при таком выборе $\delta$ все-таки может полиномиально зависеть от $N$, но так как вспомогательные задачи решаются за линейное время, то это и нестрашно: появятся лишь логарифмические множители.

Recall from Lemma \ref{lem:basic2} that the rate of convergence of AM-\ref{alg:highorder_inexact} is  $\|x_0 - x^*\|/A_k + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k$. We now finally give an estimate of $A_k$:
\begin{lemma} \label{lemma:Ak}
Suppose $H \geq 2L_f$. Then one has, with $c_1 = 4$,
\begin{align} \label{eq:Ak}
    A_k \geq \frac{k^2}{c_1 H}
\end{align}
\end{lemma}
\begin{proof}
In case, when $p = 1$ $\lambda_{k+1}$ are defined as
\begin{align*}
    \lambda_{k+1} = \frac{1}{2H}.
\end{align*}
Inequality \eqref{eq:Ak} holds when $k = 1$.

Let's proof that if \eqref{eq:Ak} holds for $k$ then it holds for $k + 1$. Using the definition of $A_k$%
\begin{align*}
    a_{k+1} = \frac{\lambda_{k+1}+\sqrt{\lambda_{k+1}^2+4\lambda_{k+1}A_k}}{2} 
\text{ , } 
A_{k+1} = A_k+a_{k+1},
\end{align*}
 we obtain
 \begin{align*}
     A_{k+1} \geq \frac{k^2}{2c_1L_f} + \frac{1}{8L_f} \left( 1 + \sqrt{1 + \frac{16k^2}{c_1}} \right) \geq \frac{(k+1)^2}{2c_1L_f}.
 \end{align*}
\
\end{proof}
\begin{proof} \textbf{of the Theorem \ref{theoremCATDinexact}}


For the first conclusion in Theorem \ref{theoremCATDinexact}, it suffices to combine Lemma \ref{lemma:Ak} with Theorem  \ref{thm:MS}.


Let's estimate solving auxiliary problems complexity. Lemma \ref{lem:ff} give us guarantees that it's sufficient to solve auxiliary problem with the accuracy \eqref{inexact_precision} in terms of criteria \eqref{eq:New_inexact}. Since auxiliary problem is every time $r$-uniformly convex we can apply \eqref{eq:lemmffF} to auxiliary problem to estimate the accuracy in terms of function discrepancy. Anyway we will have that there is no need to think about it since the dependence of this accuracy are logarithmic. The only restrictive assumption we made is that $F(x)$ is $r$-uniformly convex. 
\end{proof}


\section{Restarts}

Let's look at case when $F(x)$ admits a $(\delta, L, \mu)$ - oracle only \eqref{def:deltaLmu}.
% \pd{It would be nice to add the definition.}
Similar result to the Theorem-\ref{CATDrestarts_inexact} can be obtained in this case with minor changes.

\begin{algorithm} [h!]
\caption{AM with restarts}\label{alg:restarts_inexact_notconvex}
	\begin{algorithmic}[1]
		\STATE \textbf{Input:} $F = f + g: \R^d \rightarrow \R$ admits $(\delta, L, \mu)$ - oracle
		\STATE Set $z_0=x_0=0$ and $R_0 = \|z_0 - x_{\ast} \|$.
		\FOR{$k = 0, $ \TO $K$}
		\STATE Set $R_k=R_0\cdot 2^{-k}$ and
		\begin{equation}
		\label{numberofrestarts}
		    N_k=\max \left\{ \left\lceil \left( \frac{32 c_1 H }{\mu} \right)^{\frac{1}{2}} \right\rceil, 1\right\}.
		\end{equation}
		\STATE Set $z_{k+1} := y_{N_k}$ as the output of CATD started from $z_k$ and run for $N_k$ steps.
		\ENDFOR
		\RETURN $z_{K}$ 
	\end{algorithmic}	
\end{algorithm}

\begin{theorem}
\label{CATDrestarts_inexact}
AM with restarts for strongly convex function $F$ with constant $\mu$ converges with $N_r$ steps of AM per restart and with $N_F$ total number of AM steps, where 
% \pd{I believe here it should be $\mu$.}
\begin{equation}
    N_F = \widetilde{O} \left[\left( \frac{H R^{2-r}}{\mu} \right)^{\frac{1}{2}}\right].
\end{equation}
\end{theorem}

The proof of the theorem \ref{CATDrestarts_inexact}.
\begin{proof} 
Firstly, let's choose $\delta$ such as:
\begin{equation} \label{delta_CATD}
    \forall k: \delta + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k \leq \frac{\varepsilon}{2},
\end{equation}
where $\varepsilon$ is solution accuracy in terms of \eqref{solution accuracy}.

Then next inequality holds true
\begin{equation} \label{delta_CATD}
    \forall k: \delta + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k \leq \frac{c_1 H R^2}{k^2} .
\end{equation}


From $(\delta, L, \mu)$ - oracle definition \eqref{def:deltaLmu}
% \pd{I thought we make an assumption that it has $(\delta, L, \mu)$ - oracle rather than uniform convexity.}
 we get 
%  \pd{I'm afraid that there is a problem with the first inequality. In the case of exact oracle this inequality uses that $\la \nabla f(x^*), x- x^* \ra \geq 0$, for all $x \in Q$. Does it hold for inexact oracle?}
% \vd{Fixed.}
\begin{align} \label{RestartdeltaLmu}
     \frac{\mu}{2}\|z-x_*\|^{2} \leq F(z)-\left(F_{\delta, L,\mu}(x_*)+\left\langle \nabla F_{\delta, L,\mu}(x_*), z-x_*\right\rangle\right) = \\
      = (F(z)- F_{\delta, L,\mu}(x_*)) + \left\langle \nabla F(x_*) - \nabla F_{\delta, L,\mu}(x_*), z-x_*\right\rangle - \left\langle \nabla F(x_*), z-x_*\right\rangle \leq \\
      \leq (F(z)- F(x_*) + \delta) + \sqrt{2\delta L} \|z-x_*\|.
\end{align}
Therefore
\begin{equation}
    \frac{\mu}{2}\|z-x_*\|^{2} - \sqrt{2\delta L} \|z-x_*\| \leq (F(z)- F(x_*) + \delta).
\end{equation}
If $\delta$ is small enough such that
\begin{equation} \label{delta_CATD2}
    \frac{4\sqrt{2\delta L}}{\mu} \leq \varepsilon/2
\end{equation}
then taking into account that $\forall k: \varepsilon/2 \leq \|z_{k+1}-x_*\|$ 
% \pd{Why?} \vd{Comments added}
\begin{equation}
    \forall k: \frac{\mu}{4}\|z_{k+1}-x_*\|^{2} \geq \sqrt{2\delta L} \|z_{k+1}-x_*\|,
\end{equation}
which implies the following inequality
\begin{equation}\label{DLM:restarts}
    \frac{\mu}{4}\|z-x_*\|^{2} \leq (F(z)- F(x_*) + \delta).
\end{equation}

\begin{align*}
    R_{k+1}&=\|z_{k+1}-x_{\ast}\| \overset{\eqref{DLM:restarts}}{\leq}  \left( \frac{4 \left( F(z_{k+1})-F(x_{\ast}) + \delta \right)}{\mu} \right)^{\frac{1}{2}} \\
    &\overset{\eqref{speedCATDinexact}}{\leq}\left( \frac{4 \left( \frac{c_1 H R_k^2}{N_k^2} + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k + \delta \right)}{\mu} \right)^{\frac{1}{2}}\\
    &\overset{\eqref{delta_CATD}
    % \pd{\text{this is not clear}} \vd{\text{   seems ok now}}
    }{\leq} \left( \frac{4 \left( \frac{2 c_1 H R_{k}^{2}}{N_k^{2}} \right)}{\mu} \right)^{\frac{1}{2}} =\left( \frac{8 c_1 H R_{k}^{2}}{\mu N_k^{2}} \right)^{\frac{1}{2}}
    \overset{\eqref{numberofrestarts}}{\leq} \left( \frac{ R_{k}^{2}}{2^2 }\right)^{\frac{1}{2}} = \frac{ R_{k}}{2}.
\end{align*}
Now we compute the total number of AM steps.
\begin{align*}
    \sum\limits_{k=0}^K N_k &\leq \sum\limits_{k=0}^K \left( \frac{32 c_1 H }{\mu} \right)^{\frac{1}{2}}+K\leq \sum\limits_{k=0}^K \left( \frac{32 c_1 H }{\mu}  \right)^{\frac{1}{2}}+K\\
    &=  \left( \frac{32 c_1 H }{\mu}  \right)^{\frac{1}{2}}K+K
\end{align*}
\end{proof}

For next analysis it's advisable to obtain more practically comfortable representation of restrictions on auxiliary problem solution $\varepsilon^{(1)}$ and $\delta^{(1)}$ which appears in the definition of $(\delta^{(1)}, \mu^{(1)}, L^{(1)})$ oracle. The Theorem \ref{AM:comfortable_view} gives sufficient for convergence Algorithm \ref{alg:restarts_inexact_notconvex} conditions on $\delta^{(1)}, \varepsilon^{(1)}$.

\begin{theorem} \label{AM:comfortable_view}
Optimization problem 
\begin{equation*}
    \min_{x \in \mathbb{R}^{d_x}}F(x) = f(x)  + g(x)
\end{equation*}
is considered, where $f(x), g(x)$ are $\mu_f, \mu_g$ - strongly convex and have $L_f, L_g$ - Lipschitz continuous gradients respectively. Let also only inexact $(\delta, \mu_f, L_f), (\delta, \mu_g, L_g)$ - oracles of $f, g$ are available. 

 Then to provide $\varepsilon$-solution in terms of \eqref{speedCATDinexact} one can choose $\delta, \tilde{\varepsilon}$ such as the convergence of the Algorithm-\ref{alg:restarts_inexact_notconvex} will be performed:
 \begin{align}
    N_F = \widetilde{O} \left[\left( \frac{H R^{2-r}}{\mu} \right)^{\frac{1}{2}}\right].
\end{align}
 In addition, dependences $\delta^{(1)}(\varepsilon),\varepsilon^{(1)}(\varepsilon)$ are polynomial: 
 \begin{align}
    &\delta = \min \left\{\frac{\varepsilon \mu}{ 288^2 \cdot 2L_f},\frac{\varepsilon \mu}{ 288^2 \cdot 2L_g},  \frac{\varepsilon^{3/2}}{2 \sqrt{2 c_1 H R^2}}  \right\},\\
    & \tilde{\varepsilon} \leq \frac{\varepsilon \mu(\mu_g + H)}{144^2(L_g+H)^2}.
\end{align}
Here $L = L_f + L_g$, $\mu = \mu_f + \mu_g$. 
\end{theorem}
\begin{proof}
Firstly, let's collect all restrictions on $\delta^{(1)}$ and auxiliary problem precision for obtaining convergence of outer Algorithm-\ref{alg:restarts_inexact_notconvex} together:
\begin{align}
    \eqref{CATD:inexact_criterion}  & \|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\
    &\leq \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|-2\sqrt{2\delta L_f},\\
    \eqref{CATD:choosedelta}& \delta \leq  \frac{\varepsilon \mu}{ 32^2 \cdot L_f},\\
    \eqref{delta_CATD}&\forall k: \delta + 2\left(\sum_{i = 1}^k A_{i} \right) \delta/A_k \leq \frac{\varepsilon}{2},\\
    \eqref{delta_CATD2}& \frac{4\sqrt{2\delta L}}{\mu} \leq \varepsilon/2.
\end{align}


 Firstly, let's have a look at \eqref{CATD:inexact_criterion}. We need overwrite this condition in terms of criteria \eqref{speedCATDinexact}. 
\begin{align}
    &\|\nabla \left( \Omega_{1,\delta,L_f}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 \right)+\nabla g_{\delta,L_g}\left({y}_{k+1}\right)\|\\ 
    \leq &\|\nabla \left( \Omega_{1}\left(f, \tilde{x}_{k}, {y}_{k+1}\right)+\frac{H}{2}\left\|{y}_{k+1}-\tilde{x}_{k}\right\|^2 + g\left({y}_{k+1}\right) \right)\| + \sqrt{2 L_f \delta}+ \sqrt{2 L_g \delta}\\
    &\leq (L_g + H) \|y_{k+1} - y_{\star}\| + \sqrt{2 L_f \delta}+ \sqrt{2 L_g \delta}\\
    &\leq  (L_g + H)\sqrt{\frac{2\tilde{\varepsilon}}{H + \mu_g}} + \sqrt{2 L_f \delta}+ \sqrt{2 L_g \delta}\\
    & \leq \frac{H}{4} \|y_{k+1} - \tilde{x}_k\|.
\end{align}
Then, according to \eqref{inexact_precision}, the sufficient condition for  \eqref{CATD:inexact_criterion} holds true is:
\begin{align}
    (L_g + H)\sqrt{\frac{2\tilde{\varepsilon}}{H + \mu_g}} + \sqrt{2 L_f \delta}+ \sqrt{2 L_g \delta}
    \leq  \frac{\sqrt{\varepsilon \mu}}{72}.
\end{align}

Next \eqref{delta_CATD} is converting into more simple sufficient condition:
\begin{align}\label{choose_delta_simple_SumAi}
    &\delta \leq \frac{\varepsilon}{2\left(1 + 2 N \right)} \yad1{\leq \frac{\varepsilon}{2\left(1 + 2\left(\sum_{i = 1}^k A_{i} \right) /A_k \right)}},\\
\end{align}
where $N$ is the number of outer steps. There was used the fact that $A_{i} \leq A_{i+1}$. Finally, if $\delta$ satisfies the inequality
\begin{equation}
    \delta \leq \frac{\varepsilon^{3/2}}{2 \sqrt{2 c_1 H R^2}}
\end{equation}
then \eqref{choose_delta_simple_SumAi} holds true.

Finally, if $\delta, \tilde{\varepsilon}$ are chosen such that:
\begin{align}
    &\delta = \min \left\{\frac{\varepsilon \mu}{ 288^2 \cdot 2L_f},\frac{\varepsilon \mu}{ 288^2 \cdot 2L_g},  \frac{\varepsilon^{3/2}}{2 \sqrt{2 c_1 H R^2}}  \right\},\\
    & \tilde{\varepsilon} \leq \frac{\varepsilon \mu(\mu_g + H)}{144^2(L_g+H)^2},
\end{align}
 then all required inequalities are satisfied: 
\begin{align}
    &\frac{2(L + H)\tilde{\varepsilon}}{H + \mu_g} + \sqrt{2 L_f \delta}+ \sqrt{2 L_g \delta} \leq  \frac{\sqrt{\varepsilon \mu}}{72},\\
    & \delta \leq  \frac{\varepsilon \mu}{ 32^2 \cdot L_f},\\
     &  \delta \leq \frac{\varepsilon^{3/2}}{2 \sqrt{2 c_1 H R^2}},\\
    & \frac{4\sqrt{2\delta L}}{\mu} \leq \varepsilon/2.
\end{align}
Also dependences $\delta(\varepsilon), \tilde{\varepsilon}(\varepsilon)$ are polynomial.

\yad1{Note that $(\delta, L_{\psi}, \mu_{\psi})$ - oracle of $\psi$ can be obtained by finding $\delta/2$ --- solution of $ \max_{y \in \R^{d_y}}\underbrace{\{G(x_{k+1}^t, y)-h(y)\}}_{\psi(x)} $ \cite{Gasnikov2019}.}
\end{proof}

\newpage
\section{Список литературы}

\begin{thebibliography}{99}


\bibitem{Gasnikov2018}
\textit{ Гасников А.В.}
 Современные численные методы оптимизации. Метод
универсального градиентного спуска. М.: МФТИ, 2018.

\bibitem{Bubeck2019}
\textit{Sebastien Bubeck, Qijia Jiang, Yin Tat Lee, Yuanzhi Li, and Aaron Sidford.} Near- optimal method for highly smooth convex optimization. In Conference on Learning Theory, pages 492–507, 2019.


% \bibitem{bib_4}
% \textit{ Allen-Zhu Z., Hazan E. }
% Optimal black-box reductions between optimization
% objectives // Advances in Neural Information Processing Systems. 2016. P.
% 1614–-1622.

% \bibitem{bib_5}
% \textit{  Beznosikov A., Gorbunov E., Gasnikov A.}
% Derivative-free method for decentralized
% distributed non-smooth optimization // IFAC 2020. The 21st World Congress of the
% International Federation of Automatic Control.

% \bibitem{bib_6}
% \textit{ Bottou L., Curtis F.E., Nocedal J.}
% Optimization methods for large-scale machine
% learning // Siam Review. 2018. V. 60. No. 2. P. 223–-311.

\bibitem{Alkousa2019}
\textit{Alkousa M. et al.}
Accelerated methods for composite non-bilinear saddle point problem //  arXiv:1906.03620.

\bibitem{Baes2009}
\textit{Baes M.}
Estimate sequence methods: extensions and approximations // Institute for Operations Research, ETH, Zürich, Switzerland. – 2009.

\bibitem{Doikov2019_2}
\textit{Doikov N., Nesterov Yu.}
Nikita Doikov and Yurii Nesterov. Minimizing uniformly convex functions by cubic regularization of newton method. arXiv preprint arXiv:1905.02671, 2019.

\bibitem{Doikov2019}
\textit{Doikov N., Nesterov Yu.}
Contracting proximal methods for smooth convex optimization // arXiv:1912.07972.

\bibitem{Dvinskikh2020}
\textit{Dvinskikh D. et al.}
Accelerated and nonaccelerated stochastic gradient descent with model conception // arXiv:2001.03443

\bibitem{Dvurechensky2017}
\textit{Dvurechensky P., Gasnikov A., Tiurin A.}
 Randomized Similar Triangles Method: A
unifying framework for accelerated randomized optimization methods (Coordinate
Descent, Directional Search, Derivative-Free Method) // arXiv:1707.08486

\bibitem{Gasnikov2019}
\textit{Gasnikov A. et al.}
Near Optimal Methods for Minimizing Convex Functions with Lipschitz $p$-th Derivatives // %Conference on Learning Theory
Proceedings of the Thirty-Second Conference on Learning Theory. – 2019. – P. 1392--1393.

\bibitem{Grapiglia2019}
\textit{Grapiglia G.N., Nesterov Yu.} 
On inexact solution of auxiliary problems in tensor methods for convex optimization // arXiv:1907.13023

% \bibitem{bib_8}
% \textit{Hazan E.}
%  Lecture notes: Optimization for Machine Learning // arXiv:1909.03550

\bibitem{Ivanova2020}
\textit{Ivanova A., Gasnikov A., Dvurechensky P., Dvinskikh D., Tyurin A., Vorontsova E.,
Pasechnyuk D.}
Oracle Complexity Separation in Convex Optimization //
arXiv:2002.02706

\bibitem{Ivanova2019}
\textit{Ivanova A., Grishchenko D., Gasnikov A., Shulgin E.}
Adaptive Catalyst for smooth
convex optimization // arXiv:1911.11271

\bibitem{Kamzolov2020}
\textit{Kamzolov D., Gasnikov A., Dvurechensky P.}
On the optimal combination of tensor optimization methods // arXiv:2002.01004

\bibitem{Lan2019}
\textit{Lan G.}
 Lectures on optimization. Methods for Machine Learning //
\url{https://pwp.gatech.edu/guanghui-lan/publications/}

\bibitem{Catalyst}
\textit{Lin H., Mairal J., Harchaoui Z.}
 Catalyst acceleration for first-order convex optimization: from theory to practice //The Journal of Machine Learning Research. – 2017. – V. 18. – No. 1. – P. 7854-7907.

\bibitem{Lin2020}
\textit{Lin T., Jin C., Jordan M.} Near-optimal algorithms for minimax optimization // arXiv:2002.02417.

\bibitem{Lucchi2019}
\textit{Lucchi A., Kohler J.}
A Stochastic Tensor Method for Non-convex Optimization // arXiv:1911.10367

 \bibitem{nesterov2008accelerating}
 \textit{Nesterov Y.}
 Accelerating the cubic regularization of Newton’s method on convex problems // Mathematical Programming. – 2008. – V. 112. – №. 1. – P. 159-181.

%\bibitem{Monteiro2013}
%\textit{Monteiro R.D.C., Svaiter B.F.}
%An accelerated hybrid proximal extragradient method for convex optimization and its implications to second-order methods // SIAM Journal on %Optimization. – 2013. – V. 23. – №. 2. – P. 1092-1125.

\bibitem{NesterovImplementable}
\textit{Nesterov Yu.}
Implementable tensor methods in unconstrained convex optimization // Mathematical Programming. – 2019. – P. 1-27.


\bibitem{Nesterov2020}
\textit{Nesterov Yu.}
Inexact Accelerated High-Order Proximal-Point Methods // CORE Discussion paper 2020/8.

\bibitem{NesterovLectures}
\textit{Nesterov Yu.}
Lectures on convex optimization. Vol. 137. Berlin, Germany: Springer, 2018.

\bibitem{NesterovUnifConv}
\textit{Nesterov Yu.}
Minimizing Uniformly Convex Functions by Cubic Regularization of Newton Method

\bibitem{Gasnikov2016}
\textit{Gasnikov A.}
Searching equillibriums in large transport networks
\bibitem{Jin2020}
\textit{Tianyi Lin, Chi Jin, Michael. I. Jordan}
Searching equillibriums in large transport networks

\bibitem{AlDvinSton}
\textit{М. С. Алкуса, Д. М. Двинских, Ф. С. Стонякин}
Ускоренные методы для седловых задач

 \bibitem{bib_11}
 \textit{ Lan G., Li Z., Zhou Y.}
 A unified variance-reduced accelerated gradient method for convex optimization // Advances in Neural Information Processing Systems. – 2019. – P. 10462--10472.


\bibitem{frank_wolfe}
 \textit{ Gidel G., Jebara T.}
 Frank-Wolfe Algorithms for Saddle Point Problems
 
\bibitem{OlivierDevolder}
\textit{Olivier Devolder}
Exactness, Inexactness and Stochasticity in First-Order Methods for Large-Scale. Convex Optimization.

\bibitem{Bubeck2020}
\textit{Bubeck, S{\'e}bastien and Jiang, Qijia and Lee, Yin Tat and Li, Yuanzhi and Sidford, Aaron}
Near-optimal method for highly smooth convex optimization


% \bibitem{bib_16}
% \textit{ Nesterov Yu.}
%  Gradient methods for minimizing composite functions//
% Math. Prog.
% 2013. V.140. № 1. P. 125--161. 

% \bibitem{bib_17}
% \textit{ Nesterov Yu.}
%  Smooth minimization of non-smooth function//
% Math. Program.
% 2005. V.103. № 1. P. 127--152.

% \bibitem{bib_18}
% \textit{Shalev-Shwartz S., Ben-David S.}
%  Understanding Machine Learning: From theory to algorithms//
% Cambridge University Press.
% 2014.

% \bibitem{bib_19}
% \textit{ Shalev-Shwartz S., Shamir O., Srebro N., Sridharan K.} 
%  Stochastic Convex Optimization//
% COLT.
% 2009.



\end{thebibliography}

